Voluntary Retreat for Decentralized Interference Reduction in Robot Swarms

In densely-packed robot swarms operating in confined regions, spatial interference -- which manifests itself as a competition for physical space -- forces robots to spend more time navigating around each other rather than performing the primary task. This paper develops a decentralized algorithm that enables individual robots to decide whether to stay in the region and contribute to the overall mission, or vacate the region so as to reduce the negative effects that interference has on the overall efficiency of the swarm. We develop this algorithm in the context of a distributed collection task, where a team of robots collect and deposit objects from one set of locations to another in a given region. Robots do not communicate and use only binary information regarding the presence of other robots around them to make the decision to stay or retreat. We illustrate the efficacy of the algorithm with experiments on a team of real robots.

==> sections/prob_form.tex <==
 
%Assuming homogeneous circular robots having radius $\epsilon_r$, the only interactions between the robots occur in the form of {\it encounters}, where robot $i$ encounters $j$ at time $t_e$ if $\| x_i(t_e) - x_j(t_e) \| \leq 2\epsilon_r$ and if there exists a $t<t_e$, such that $\| x_i(t) - x_j(t) \| > 2\epsilon_r$. Note that although apparently cumbersome at first, this definition is necessary because, in reality, encounters are discrete-time events separated by finite time intervals. 

%We let $P(t)$ be the number of tasks available in the domain at time $t$, and $p_k(t)$, for $k=1,\dots,P(t)$, denotes the position of $k^{\text{th}}$ task's center. We model tasks as homogeneous discs of radius $\epsilon_p$ uniformly distributed at random on $\mathcal{D}$. We assume new tasks to be continuously added to the domain. We model the generation of new tasks as a Poisson process with constant intensity $\lambda_{p}$, where $\lambda_{p}$ is the average number of tasks generated per unit of time. 

